World Discovery Models

As humans we are driven by a strong desire for seeking novelty in our world. Also upon observing a novel pattern we are capable of refining our understanding of the world based on the new information---humans can discover their world. The outstanding ability of the human mind for discovery has led to many breakthroughs in science, art and technology. Here we investigate the possibility of building an agent capable of discovering its world using the modern AI technology. In particular we introduce NDIGO, Neural Differential Information Gain Optimisation, a self-supervised discovery model that aims at seeking new information to construct a global view of its world from partial and noisy observations. Our experiments on some controlled 2-D navigation tasks show that NDIGO outperforms state-of-the-art information-seeking methods in terms of the quality of the learned representation. The improvement in performance is particularly significant in the presence of white or structured noise where other information-seeking methods follow the noise instead of discovering their world.

==> generalsetting.tex <==
\section{Notations and Background}
\label{sec:general setting}

\paragraph{Partially observable setting.} We consider a partially observable environment where an agent get some observation $o_t$ at time $t$, then selects and action $a_t$, which generates a new observation $o_{t+1}$ at the next time step. We assume observations $o_t$ are coming from some underlying process $x_t$ with Markov dynamics, i.e.~$x_{t+1} \sim P(\cdot |x_t,a_t)$, where $P$ is the dynamics of the underlying process. This setting can be formalised with Partially Observable Markov Decision Processes~\citep[POMDPs;][]{lovejoy1991survey,cassandra1998exact}. In other words, the observation $o_t$ gives incomplete information about the real state $x_t$ which represents what is to know about the world at time $t$ in order to predict the future. Thus, the agent has an uncertainty on the real state $x_t$ as well as on the next state $x_{t+1}$ as the dynamics depends on the state-action pair $(x_t, a_t)$. Therefore, a key problem in POMDPs is  to maintain a belief state, a distribution on the real states, quantifying the uncertainty on the identity of $x_t$ given the history of previous observations-actions $h_t$.

More formally, at a given time $t$, the current history $h_t$ is the set of past actions and observations
\begin{equation}\label{eq:hist}
h_t \eqdef \{o_0, a_0, o_1, a_1, \cdots, a_{t-1}, o_t\},
\end{equation}
and a belief $P_b(\cdot|h_t)$ is a distribution over the possible states conditioned on the history of past actions and observations. A belief distribution represents therefore the actual knowledge of the agent about the world. Learning a belief state directly using the existing architectures is not an easy job, especially in the self-supervised regime. Instead following~\citep{guo2018} one can learn efficiently an internal representation or an encoding of the history $b_t=f(h_t)$. This representation can then be evaluated in terms of its accuracy in estimating the real belief (see Sec.~\ref{subsec:Evaluation}).  



\paragraph{Information gain.} A very broad definition of the information gain~\citep{schmidhuber2010formal} is the distance or divergence between distributions on any  random event of interest $\Omega$ before and after a new sequence of observations. The random event can be the parameters of the modelled dynamics (Bayesian surprise) or future observations or actions. Various distances or divergences also could be considered such as Shannon-Jensen divergence or Wasserstein distance, but in the literature of intrinsic motivation, the Kullback-Leibler divergence is mostly chosen to define the information gain. Here we use the \emph{predictive information gain}, which is the information gain w.r.t. the future observation (i.e., $\Omega=o_{t+k}$ for every $k\geq1$ and $t\geq 0$).


Let $t\geq0$  and $k\geq1$ be some integers. Let $\A_{t,k}\eqdef \{a_t,\dots,a_{t+k-1}\}$  and $\mathcal O_{t,k}\eqdef \{o_t,\dots,o_{t+k-1}\}$ be the sequence of actions and observations from time $t$ up to time $t+k-1$, respectively. Let $\mathbb{P}(o_{t+k}|h_{t}, \A_{t,k})$ be the probability of observing $o_{t+k}$ given the history $h_t$ and the sequence of actions $\A_{t,k}$, where $h_t$ is defined from \cref{eq:hist}. For conciseness  we use the short-hand notation $\mathbb{P}_{t, k}=\mathbb{P}(o_{t+k}|h_t, \A_{t,k}) $ when no confusion is possible. Then the $k$-step predictive information gain $IG(o_{t+k}, \mathcal O_{t,k}|h_t, \A_{t,k})$ of the future event $o_{t+k}$ with respect to the sequence of observations $\mathcal O_{t,k}$ is defined as:
\begin{align}
IG(o_{t+k}, \mathcal O_{t,k}|h_t, \A_{t,k}) \eqdef KL\left(\mathbb{P}_{t, k} || \mathbb{P}_{t-1, k+1} \right),
\end{align}
 In the case $k=1$ we recover the 1-step information gain on the next observation $o_{t+1}$ due to $o_t$. We also use the following short-hand notation for the information gain $IG_{t, k} = IG(o_{t+k}, \mathcal O_{t,k}|h_t, \A_{t,k})$ for every $k\geq 1$ and $t\geq0$. Also by convention we define $IG_{t, 0}=0$. 



Other types of information gain have been considered previously~\citep{houthooft2016vime, little2013learning, achiam2017surprise} in a fully-observable setting. In this framework, the information gain corresponds on how much the new observation $o_t$ can refine the posterior on probability distribution over the entire model dynamics $P$ of the system. There the parameters of dynamics $P$ are seen as a random variable that is updated with new observations. This works in tabular state-action space~\citep{little2013learning} where one can easily parameterise a model of the dynamics and compute a posterior upon receiving the new observation. However, when using neural networks, ~\citet{houthooft2016vime} showed that computing the posterior becomes intractable and therefore some approximations (variational lower bound) is used for optimisation. We argue that choosing a simpler notion of predictive information gain allows us to compute easily the prior and posterior distributions with neural networks which makes our method tractable and not relying on approximations. 

\paragraph{Information gain2.} A very broad definition of the information gain~\citep{schmidhuber2010formal} is the distance or divergence between distributions on any  random event of interest $\Omega$ before and after a new sequence of observations. The random event can be the parameters of the modelled dynamics (Bayesian surprise) or future observations or actions. Various distances or divergences also could be considered such as Shannon-Jensen divergence or Wasserstein distance, but in the literature of intrinsic motivation, the Kullback-Leibler divergence is mostly chosen to define the information gain. 

Choosing $\Omega=o_{t+k}$ for every $k\geq1$ and $t\geq 0$, the information gain is

Let $t\geq0$  and $k\geq1$ be some integers. Let $\A_{t,k}\eqdef \{a_t,\dots,a_{t+k-1}\}$  and $\mathcal O_{t,k}\eqdef \{o_t,\dots,o_{t+k-1}\}$ be the sequence of actions and observations from time $t$ up to time $t+k-1$, respectively. Let $\mathbb{P}(o_{t+k}|h_{t}, \A_{t,k})$ be the probability of observing $o_{t+k}$ given the history $h_t$ and the sequence of actions $\A_{t,k}$, where $h_t$ is defined from \cref{eq:hist}. For conciseness  we use the short-hand notation $\mathbb{P}_{t, k}=\mathbb{P}(o_{t+k}|h_t, \A_{t,k}) $ when no confusion is possible. Then the $k$-step predictive information gain $IG(o_{t+k}, \mathcal O_{t,k}|h_t, \A_{t,k})$ of the future event $o_{t+k}$ with respect to the sequence of observations $\mathcal O_{t,k}$ is defined as:
\begin{align}
IG(o_{t+k}, \mathcal O_{t,k}|h_t, \A_{t,k}) \eqdef KL\left(\mathbb{P}_{t, k} || \mathbb{P}_{t-1, k+1} \right),
\end{align}
 In the case $k=1$ we recover the 1-step information gain on the next observation $o_{t+1}$ due to $o_t$. We also use the following short-hand notation for the information gain $IG_{t, k} = IG(o_{t+k}, \mathcal O_{t,k}|h_t, \A_{t,k})$ for every $k\geq 1$ and $t\geq0$. Also by convention we define $IG_{t, 0}=0$. 


Other types of information gain have been considered previously~\citep{houthooft2016vime, little2013learning, achiam2017surprise} in a fully-observable setting. In this framework, the information gain corresponds on how much the new observation $o_t$ can refine the posterior on probability distribution over the entire model dynamics $P$ of the system. There the parameters of dynamics $P$ are seen as a random variable that is updated with new observations. This works in tabular state-action space~\citep{little2013learning} where one can easily parameterise a model of the dynamics and compute a posterior upon receiving the new observation. However, when using neural networks, ~\citet{houthooft2016vime} showed that computing the posterior becomes intractable and therefore some approximations (variational lower bound) is used for optimisation. We argue that choosing a simpler notion of predictive information gain allows us to compute easily the prior and posterior distributions with neural networks which makes our method tractable and not relying on approximations. 


==> guideline.tex <==
We consider a partially observable environment where an agent get some observation $o_t$ at time $t$, then selects and action $a_t$, which generates a new observation $o_{t+1}$ at the next time step.

We assume observations $o_t$ are coming from some underlying process $x_t$ with Markov dynamics, i.e.~$x_{t+1} \sim p(\cdot |x_t,a_t)$, where $p$ is dynamics of the underlying process.

We are interested in the possibility to learn a representation $h_t=f(H_t)$, function of the history ($H_t = \{o_s\}_{s\leq t}\cup \{a_s\}_{s< t}$, i.e., all previous observations and actions), that would encode some properties of the ground truth state $x_t$.



\todo{remi: Talk about POMDP here}. However here we do not assume that the agent knows anything about the underlying process $x_t$ neither about its dynamics $p$.


It is well known that Predictive State Representation (PSR, reference here) is a set of core predictors which form a sufficient statistics for predicting any future observation $o_{t+k}$ given any sequence of actions $a_{t:t+k-1}$ and history $H_t$. Indeed, the (Hankel) matrix of infinite by infinite dimension of all probabilities of any sequence of observations conditioned on any sequence of actions and any history is of rank at most $n$, where $n$ is the number of states of the underlying Markov process. 

[Guo et al, 2018] showed that an agent equipped with a recurrent network trained to make predictions of future observations, conditioned on actions, can learn a representation which encodes a distribution over the ground truth state. They used a contrastive loss (Contrastive Predicting Coding [Ref here]) to avoid having to generate the future frame, which may be too complex in visually rich environments like DM Lab [ref here]. However the policy used for making the predictions was hand-designed. It was not learnt. 

However the PSR result says that we can get sufficient statistics when predicting future observations corresponding to {\em any} possible sequence of actions. But it is clear that some sequences are better than others in terms of the quality of the learnt representation. Indeed, it may be very easy to predict future observations when an agent in a room keeps moving against a wall (since the observations does not change), but by doing so, the agent does not learn anything about the room it is in. These predictions are easy but not informative. Whereas other predictions, such as what  the agent would see if it would turn around (basically predict what is in its back), may be harder to make but will reveal more information to learn from, thus potentially improving the quality of the representation $h_t$.

The goal of this paper is to investigate what are the best sequences of actions -for which the agent will learn the most- when asked to predict future observations conditioned on these actions. One can see this problem in a similar way as the way a scientist  develops and refines its model of the world. At some point in time, he possesses a current model of the world (ability to predict future observations conditioned on actions). Now he wants to improve this model, so he will set up an {\em experiment} in order to validate or invalidate the current model. Then he executes the experiment and update the model according to the outcome. In our case the experiment is a sequence of actions. Our agent will select a sequence of actions (an experiment). Before acting, the agent makes a prediction of the resulting observation based on its current model. Then it executes the sequence of actions and it observes the outcome. Finally it refines its model accordingly to how well it matches its prediction.

So our goal is to train an agent to design  experiments (sequence of actions) in order to refine its model of its world, in order to learn as much as possible the dynamics of the world it is in. 

We will use an adversarial approach where the agent will be encourage to go to places of the environment in order to make the most difficult predictions -but from which it can learn something. We are training a {\em scientist agent.}


%\paragraph{Motivation for information-seeking agents.}
% NDIGO seeks information about the agent position.
% Support: Fork experiment, compared to epsilon-greedy exploration.
% Measure: Average indicator that agent reaches the end of the hallway in each episode, versus episode number (throughout training).
% As a start, to motivate the kind of information-seeking behaviour we can obtain with NDIGO, we will present an experiment where we trained our NDIGO agent in the \fork{} environment.
% The environment is shown in \cref{fig:forkEnvironment}, and consists of a gridworld\footnote{
%     The gridworld environments in this paper are implemented using the \texttt{pycolab} library, available at \url{https://github.com/deepmind/pycolab}.
% } room with three hallways connected at the near end.
% Each episode, the agent starts in the far end of one of the hallways, with equal probability.
% The environment is partially observable: At any given time the agent only sees the $5 \times 5$ region centred on it, so it is not possible to distinguish the hallways except at the near end of the room.
% \Cref{fig:forkPerformance} shows that the trained NDIGO agent consistently goes to the near end of the room, where the position of the agent can be resolved.
% It is worth remarking that \citet{guo2018} have shown that the representation learned by NDIGO encodes the position of the agent as well as uncertainty\footnote{
%     To be precise, the representation encodes enough information to parameterise an accurate belief over the agent's position \citep{guo2018}.
% }, and \cref{fig:forkPerformance} indicates that NDIGO agents are able to act in the environment to reduce this uncertainty.
% %
% \begin{figure}
%     \centering
%     \includegraphics[width=4cm, draft]{stub}
%     \caption{Top-down view of the \fork{} environment.
%     \label{fig:forkEnvironment}}
% \end{figure}
% %
% \begin{figure}
%     \centering
%     \includegraphics[width=4cm, draft]{stub}
%     \caption{
%     Average indicator that the agent reaches the near end of the room in the episode for NDIGO, PE and PG, versus training step.
%     \label{fig:forkPerformance}}
% \end{figure}



% \paragraph{Comparing NDIGO and baselines on information-seeking behaviour.}
% \paragraph{Claim:} NDIGO \& PE seek information about objects that change each episode. PG does not.
% Support: 5 rooms with object in one of the rooms.
% Measure: Average indicator that agent sees the object in an episode, versus episode number (throughout training). Perhaps also looking at the fist spotting time.


% \paragraph{Representation Stability}
% \paragraph{Claim:} Our representation allows keeping track of periodic movements. Once the agent sees the bouncing, its location can be accurately predicted even when the agent has moved away.
% Support: 5 rooms with bouncing in 1-4, but bouncing has to be different from episode to episode.
% Measure: We have to track the misclassification error of the layout predictor for the bouncing objects.


